Do Vision-Language Models Represent Space and How? Evaluating Spatial Frame of Reference Under Ambiguities

Spatial expressions in situated communication can be ambiguous, as their meanings vary depending on the frames of reference (FoR) adopted by speakers and listeners. While spatial language understanding and reasoning by vision-language models (VLMs) have gained increasing attention, potential ambiguities in these models are still under-explored. To address this issue, we present the COnsistent Multilingual Frame Of Reference Test (COMFORT), an evaluation protocol to systematically assess the spatial reasoning capabilities of VLMs. We evaluate nine state-of-the-art VLMs using COMFORT. Despite showing some alignment with English conventions in resolving ambiguities, our experiments reveal significant shortcomings of VLMs: notably, the models (1) exhibit poor robustness and consistency, (2) lack the flexibility to accommodate multiple FoRs, and (3) fail to adhere to language-specific or culture-specific conventions in cross-lingual tests, as English tends to dominate other languages. With a growing effort to align vision-language models with human cognitive intuitions, we call for more attention to the ambiguous nature and cross-cultural diversity of spatial reasoning.

==> floating/fig-convention_case_study.tex <==
\begin{wrapfigure}{!tr}{0.55\textwidth}
    \centering
    \begin{subfigure}[t]{.2\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/metrics_deviation_angle.pdf}
        \caption{The conventional left in English has a deviation angle $\theta = 90\degree$ relative to the conventional front.}
        \label{fig:metric-angle}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/metric_normalization.pdf}
        \caption{The raw probability curve $p(\theta)$ in gray, normalized probability curve $\widehat{p}(\theta)$ in black, and two reference probability curves $p_\textrm{hemi}(\theta)$ and $p_\textrm{cos}(\theta)$ in red and purple.}
        \label{fig:metric-curve}
    \end{subfigure}   
    \vspace*{-5pt}
    \caption{An illustration of the performance metrics. \vspace*{-5pt}}
    \label{fig:metric-error}
\end{wrapfigure}

==> floating/fig-metric.tex <==
\begin{wrapfigure}{!tr}{0.5\textwidth}
    \centering  
    \vspace*{-10pt}
    \begin{subfigure}[t]{.2\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/metrics_deviation_angle.pdf}
        \caption{The red ball (to the conventional left of the blue ball in English) has a deviation angle $\theta = 90\degree$ relative to the conventional front.}
        \label{fig:metric-angle}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.27\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/metric_normalization.pdf}
        \caption{The raw probability curve $p(\theta)$ in gray, normalized probability curve $\widehat{p}(\theta)$ in black, and two reference probability curves $p_\textrm{hemi}(\theta)$ and $p_\textrm{cos}(\theta)$ in purple and red.}
        \label{fig:metric-curve}
    \end{subfigure}   
    \vspace*{-5pt}
    \caption{An illustration of the performance metrics. \vspace*{-5pt}}
    \label{fig:metric-error}
\end{wrapfigure}

==> floating/fig-preferredfor_analysis_case_study.tex <==
\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.25\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/CAR_all_plots/nop/LLaVA1.513B/front.pdf}%{plots/CAR_lineplot/nop/llava-v1.5-13b/Is the [A] in front of the [B]__err_0.34951568531037774.pdf}
    \caption{LLaVA-1.5-13B: \\In front of}
    \label{fig:Is the [A] in front of the [B]__err_0.34951568531037774}
  \end{subfigure}
  \hspace{0.05\columnwidth}
  \begin{subfigure}[b]{0.25\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/CAR_all_plots/nop/GPT4o/behind.pdf}%{plots/CAR_lineplot/nop/GPT-4o/Is the [A] behind the [B]__err_0.4024524538725301.pdf}
    \caption{GPT-4o: \\Behind}
    \label{fig:Is the [A] behind the [B]__err_0.4024524538725301}
  \end{subfigure}
  \caption{Preferred FoR and language ambiguity}
  \label{fig:convention_shift}
\end{figure}

==> floating/fig-symm.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/metrics_sym.pdf}
    \vspace*{-20pt}
    \caption{An illustration of the spatial symmetry with respect to the front. As the red sphere rotates around the blue sphere, the spatial symmetry metric ensures that the symmetric pairs, \(\theta\) and \(-\theta\), have the same probability of being identified as the front. \vspace*{-5pt}}
    \label{fig:metric-sym}
\end{figure}

==> floating/tab-prompt.tex <==
\begin{wraptable}{tr}{0.45\textwidth}
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{0.8}
    \centering
    \begin{tabular}{C{0.9cm}C{5.2cm}}
        \toprule
        \textbf{Origin} & \textbf{Prompt Template} \\
        \midrule
        nop & Is \texttt{[A]} \texttt{[relation]} \texttt{[B]}? \\
        \midrule
        cam & From the camera's viewpoint,\newline is \texttt{[A]} \texttt{[relation]} \texttt{[B]}? \\
        \midrule
        add & From the \texttt{[addressee]}'s viewpoint,\newline is \texttt{[A]} \texttt{[relation]} \texttt{[B]}? \\
        \midrule
        rel & From the \texttt{[relatum]}'s viewpoint,\newline is \texttt{[A]} \texttt{[relation]} \texttt{[B]}? \\
        \bottomrule
    \end{tabular}
    \caption{The origins of each reference system and the corresponding prompt templates for querying a target-relation-reference triple. \vspace*{-5pt}}
    \label{tab:prediction_notation}
\end{wraptable}

==> floating/tab-removed-languages.tex <==
\begin{table}
\centering
    \begin{tabular}{cc}
    \hline
    Code & Language \\
    \hline
    ay & Aymara \\
    bm & Bambara \\
    hr & Croatian \\
    dv & Dhivehi \\
    doi & Dogri \\
    ee & Ewe \\
    gn & Guarani \\
    hmn & Hmong \\
    ky & Kyrgyz \\
    lg & Luganda \\
    ml & Malayalam \\
    mni-Mtei & Meiteilon (Manipuri) \\
    lus & Mizo \\
    or & Odia (Oriya) \\
    pa & Punjabi \\
    qu & Quechua \\
    sm & Samoan \\
    tt & Tatar \\
    te & Telugu \\
    ti & Tigrinya \\
    ug & Uyghur \\
    xh & Xhosa \\
    yo & Yoruba \\
    \hline
    \end{tabular}
    \caption{A list of 23 languages that are removed from our multilingual evaluation because they are not following instructions of generating predictions of 'yes' and 'no'.}
    \label{tab:list_removed_languages}
\end{table}
